DeepMill: Neural Accessibility Learning for Subtractive Manufacturing

Manufacturability is vital for product design and production, with accessibility being a key element, especially in subtractive manufacturing. Traditional methods for geometric accessibility analysis are time-consuming and struggle with scalability, while existing deep learning approaches in manufacturability analysis often neglect geometric challenges in accessibility and are limited to specific model types. In this paper, we introduce DeepMill, the first neural framework designed to accurately and efficiently predict inaccessible and occlusion regions under varying machining tool parameters, applicable to both CAD and freeform models. To address the challenges posed by cutter collisions and the lack of extensive training datasets, we construct a cutter-aware dual-head octree-based convolutional neural network (O-CNN) and generate an inaccessible and occlusion regions analysis dataset with a variety of cutter sizes for network training. Experiments demonstrate that DeepMill achieves 94.7% accuracy in predicting inaccessible regions and 88.7% accuracy in identifying occlusion regions, with an average processing time of 0.04 seconds for complex geometries. Based on the outcomes, DeepMill implicitly captures both local and global geometric features, as well as the complex interactions between cutters and intricate 3D models.

==> figures/fig-Ablation-study.tex <==
\begin{figure}[t]
%\vspace{-5pt}
\centering
  \includegraphics[width=1.0\linewidth]{images/Ablation-study.png}
	% \vspace{-15pt}
\caption{Given the initial....}
  \label{fig:Ablation-study}    
\end{figure}

==> figures/fig-Comparison-cutter-module.tex <==
\begin{figure}[t]
%\vspace{-5pt}
\centering
  \includegraphics[width=1.0\linewidth]{images/Comparison-cutter-module.png}
	% \vspace{-15pt}
\caption{Given the initial....}
  \label{fig:Comparison-cutter-module}    
\end{figure}

==> figures/fig-Complex-models.tex <==
\begin{figure}[t]
%\vspace{-5pt}
\centering
  \includegraphics[width=1.0\linewidth]{images/Complex-models.png}
	% \vspace{-15pt}
\caption{Given the initial....}
  \label{fig:Complex-models}    
\end{figure}

==> figures/fig-GraphSAGE.tex <==
\begin{figure}[t]
%\vspace{-5pt}
\centering
  \includegraphics[width=1.0\linewidth]{images/GraphSAGE.png}
	% \vspace{-15pt}
\caption{Given the initial....}
  \label{fig:GraphSAGE}    
\end{figure}

==> figures/fig-gallery.tex <==
\begin{figure*}[htbp]
%\vspace{-5pt}
\centering
  \includegraphics[width=1.0\linewidth]{images/gallery.png}
	% \vspace{-15pt}
\caption{Given the initial....}
  \label{fig:gallery}    
\end{figure*}

==> figures/fig-pipeline.tex <==
\begin{figure*}[t]
%\vspace{-5pt}
\centering
  \includegraphics[width=1.0\linewidth]{images/pipeline.png}
	% \vspace{-15pt}
\caption{Given the initial....}
  \label{fig:pipeline}    
\end{figure*}

==> figures/fig-symmetry.tex <==
\begin{figure}[t]
\centering
  \includegraphics[width=1.0\linewidth]{images/symmetry.png}
	% \vspace{-15pt}
\caption{Given the initial....}
  \label{fig:symmetry}    
\end{figure}

==> tables/table-evaluation.tex <==

\begin{table}[t]
\renewcommand{\arraystretch}{1.0}
\centering
\caption{ 
Program running time of each step (second).
$Ori$ is the time to determine the setup of $M^*$.
$Pre$ is the time of Pre-processing.
$Ini$ represents the time of initialization of clipping planes.
$MCTS$ is the time of the Monte Carlo Tree Search.
$Pos$ represents the post-processing time for generating AM positional blocks.
$T$ is the total running time (minute).
}
\begin{tabular}{m{1.8cm}<{\centering}| m{0.65cm}<{\centering}  m{0.5cm}<{\centering} m{0.5cm}<{\centering} m{0.7cm}<{\centering} m{0.6cm}<{\centering} |m{0.8cm}<{\centering} }
\hline
{Model} 
& \centering{$Ori$} 
& \centering{$Pre$}
& \centering{$Ini$}
& \centering{$MCTS$} 
& \centering{$Pos$} 
& {$T$} \\
\hline
%\rule{0pt}{15pt}
{Bearing}     &{166} &{9} &{13} &{194} &{2} &{6.4} \\
\hline
{Hand}     &{215} &{37} &{22} &{527} &{5} &{13.4} \\
\hline
{Coral}     &{114} &{11} &{69} &{157} &{4} &{5.9} \\
\hline
{Bracket}     &{111} &{56} &{8} &{401} &{4} &{9.7} \\
\hline
{Holder}     &{92} &{18} &{10} &{220} &{5} &{5.8} \\
\hline
{Opener}     &{145} &{24} &{27} &{415} &{81} &{11.5} \\
\hline
{Impeller}     &{197} &{37} &{8} &{510} &{37} &{13.2} \\
\hline
{Sculpture}     &{195} &{17} &{38} &{240} &{6} &{8.3} \\
\hline
{Prince}     &{205} &{9} &{9} &{134} &{2} &{6.0} \\
\hline
{Cow}     &{63} &{6} &{2} &{81} &{1} &{2.6} \\
\hline
{Swan}     &{178} &{21} &{21} &{399} &{8} &{10.5} \\
\hline
{Tree}     &{157} &{17} &{52} &{88} &{8} &{5.4} \\
\hline
\end{tabular}
\label{table:runtime}
\end{table}

